Novel Region of Attraction Characterization for Control and Stabilization of Voltage Dynamics

In this paper, we study the monitoring and control of long-term voltage stability considering load tap-changer (LTC) dynamics. We show that under generic conditions, the LTC dynamics always admit a unique stable equilibrium. For the stable equilibrium, we characterize an explicit inner approximation of its region of attraction (ROA). Compared to existing results, the computational complexity of the ROA characterization is drastically reduced. A quadratically constrained linear program formulation for the ROA characterization problem is proposed. In addition, we formulate a second-order cone program for online voltage stability monitoring and control exploiting the proposed ROA characterization, along with an ADMM-based distributed algorithm to solve the problem. The efficacy of the proposed formulations and algorithms is demonstrated using a standard IEEE test system.

==> Two-Bus.tex <==
\section{Two-Bus System Model} \label{sect:2bus}

We use a simple two-bus system model to illustrate the basic idea of our analysis on dynamics and stability of LTC. 
The continuous approximation of the discrete LTC dynamics is given as follows \cite{van2007voltage}
\begin{align} \label{eq:LTCdyn}
    T \dot{r} = V(r) - V_0,
\end{align}
where $T$ is the time constant, $r$ is the tap ratio, $V(r)$ is the controlled voltage magnitude on the secondary side of the LTC and $V_0$ is the given reference voltage magnitude.

Consider a two-bus system where bus 1 is a generator bus with constant voltage $\tilde{E} = E e^{j0}$, bus 2 is a load bus with voltage $\tilde{V}_1 = V_1e^{j\theta}$, and the two buses are connected through a transmission line with impedance $\tilde{Z} = R + jX$. The load at bus 2 is modeled as a constant admittance load with admittance $\tilde{Y}_L = G_L + jB_L$ behind an LTC with tap ratio $r:1$. For brevity, denote the magnitudes of line impedance and load admittance by $Z$ and $Y_L$, respectively. In addition, let $\tilde{V}_2 = V_2e^{j\theta}$ denote the voltage on the secondary side of the LTC, and so we have $\tilde{V}_1 / \tilde{V}_2 = r$.

By Kirchhoff's current law at bus 2, we have
\begin{align} \label{eq:KCL:2bus}
    \frac{\tilde{E} - \tilde{V}_1}{\tilde{Z}} = \frac{\tilde{V}_1}{r^2 / \tilde{Y}_L}.
\end{align}
After simple manipulations, solving for $\tilde{V}_1$ gives
\begin{align}
    \tilde{V}_1 = \frac{r^2 \tilde{E}}{\tilde{Z}\tilde{Y}_L + r^2}.
\end{align}
It follows from $\tilde{V}_1 / \tilde{V}_2 = r$ that
\begin{align}
    \tilde{V}_2 = \frac{\tilde{V}_1}{r} = \frac{r \tilde{E}}{\tilde{Z}\tilde{Y}_L + r^2}.
\end{align}
If we denote the reference voltage magnitude of the LTC by $V_0$, then we know from \eqref{eq:LTCdyn} that at an equilibrium point of \eqref{eq:LTCdyn} $V_2 = V_0$, or
\begin{align} \label{eq:V2=V0}
    \left| \frac{r \tilde{E}}{\tilde{Z}\tilde{Y}_L + r^2} \right| = V_0.
\end{align}
After some algebraic manipulations, \eqref{eq:V2=V0} can be rewritten as the following quadratic equation in $r^2$:
\begin{align} \label{eq:quartic}
    V_0^2 r^4 + \left( 2V_0^2(RG_L - XB_L) - E^2 \right) r^2 + V_0^2Y_L^2Z^2 = 0.
\end{align}
Let the coefficients and discriminant of the quadratic equation \eqref{eq:quartic} be $a, b, c$, and $\Delta$, respectively. That is
\begin{subequations} \label{eq:abcd}
\begin{align}
    a &:= V_0^2,\\
    b &:= 2V_0^2(RG_L - XB_L) - E^2,\\
    c &:= V_0^2Y_L^2Z^2, \\
    \Delta &:= b^2 - 4ac.
\end{align}
\end{subequations}
Since $a, c \ge 0$, \eqref{eq:quartic} admits a nonnegative solution $r^2$ if and only if
\begin{align} \label{eq:condition:r}
    \Delta \ge 0 \text{ and } b \le 0.
\end{align}
For any given $\tilde{Y}_L$ that satisfies \eqref{eq:condition:r}, there are two equilibrium points for the LTC dynamics \eqref{eq:LTCdyn} given by
\begin{align} \label{eq:equilibrium}
    r_\pm &= \sqrt{\frac{-b \pm \sqrt{\Delta}}{2a}}.
\end{align}
It can be verified that $V_2(r) \ge V_0$ if and only if $r_- \le r \le r_+$, which implies $r_+$ is a stable equilibrium and $r_-$ is unstable, and the ROA is $\{r:\; r \ge r_- \}$. We demonstrate this through numerical examples below.

\subsection{Example 1}

Suppose we have a lossless two-bus system with the following parameters: $E = X = 1$, $R = 0$. Further suppose the load is capacitive with constant power factor: $G_L = 2B_L \ge 0$. For this system the quantities in \eqref{eq:abcd} are
\begin{subequations}
    \begin{align}
        a &= 1, \\
        b &= -(2B_L + 1), \\
        c &= 5B_L^2, \\
        \Delta &= -16B_L^2 + 4B_L + 1.
    \end{align}
\end{subequations}
We see that $b \le 0$ always holds as $B_L \ge 0$, so condition \eqref{eq:condition:r} is satisfied when $\Delta \ge 0$, which is $B_L \le (1 + \sqrt{5})/8 \approx 0.4045$. The equilibrium points for various load admittance values ($B_L$-$r$ curve) are plotted in Fig. \ref{fig:br}. 

Suppose the load admittance is $\tilde{Y}_L = 0.8 + j0.4$. The two equilibria given by \eqref{eq:equilibrium} are $r_+ = 1$ and $r_- = 2\sqrt{5}/5 \approx 0.8944$. We know from preceding discussion that the system \eqref{eq:LTCdyn} will be stabilized and the trajectory converges to $r_+$ when $r > r_-$. This is demonstrated in Fig. \ref{fig:dynamics}, where the LTC is initialized at $r(t = 0) = 0.9$ and $r(t = 0) = 0.89$, respectively. It is seen that the trajectory converges to $r_+ = 1$ for $r(t = 0) = 0.9$ but fails to do so when the initial value is less than the threshold $r(t = 0) = r_-$.

\begin{figure}[!t]
	\centering
	\includegraphics[width=3.4in]{br.jpg}
	% where an .eps filename suffix will be assumed under latex, 
	% and a .pdf suffix will be assumed for pdflatex; or what has been declared
	% via \DeclareGraphicsExtensions.
	\caption{Tap ratios at equilibrium for various susceptance values.}
	\label{fig:br}
\end{figure}

\begin{figure}[!t]
	\centering
	\includegraphics[width=3.4in]{dynamics.jpg}
	% where an .eps filename suffix will be assumed under latex, 
	% and a .pdf suffix will be assumed for pdflatex; or what has been declared
	% via \DeclareGraphicsExtensions.
	\caption{LTC dynamics at different initial points. Time constant $T = 1$.}
	\label{fig:dynamics}
\end{figure}


\subsection{Example 2}

In the second example, we examine the effect of stabilizing the post-fault LTC dynamics via demand side support.

Suppose the system parameters are identical to those in the last example initially. To model line tripping, we increase the transmission line reactance by $20\%$ so that the post-fault $X' = 1.2$. The comparison between the $B_L$-$r$ curves before and after the event is shown in Fig. \ref{fig:br2}. It is seen that the event reduces the critical admittance value and the maximal power demand. In particular, we see that the original load admittance $0.8 + j0.4$ is no longer feasible and will lead to voltage collapse if no countermeasures are taken. 

The LTC dynamics are shown in Fig. \ref{fig:dynamics2}. The system is initially at steady state with steady-state tap ratio $r = 1$. The line tripping happens at time $t = 10$, which leads to the initial decline of secondary side voltage, which is then exacerbated by the LTC dynamics \eqref{eq:LTCdyn}. Without any countermeasures, the system collapses, as shown by the solid blue line in Fig. \ref{fig:dynamics2}. However, if we initiate demand side support by injecting power at the secondary side $1$ second after the fault, which is modeled by decreasing both the load conductance and susceptance by $30\%$, we see that the system can be brought back to steady state as shown in the dashed red line in Fig. \ref{fig:dynamics2}. 

\begin{figure}[!t]
	\centering
	\includegraphics[width=3.4in]{br2.jpg}
	% where an .eps filename suffix will be assumed under latex, 
	% and a .pdf suffix will be assumed for pdflatex; or what has been declared
	% via \DeclareGraphicsExtensions.
	\caption{Tap ratios at equilibrium for various susceptance values for the original case and after line tripping event.}
	\label{fig:br2}
\end{figure}

\begin{figure}[!t]
	\centering
	\includegraphics[width=3.4in]{dynamics2.jpg}
	% where an .eps filename suffix will be assumed under latex, 
	% and a .pdf suffix will be assumed for pdflatex; or what has been declared
	% via \DeclareGraphicsExtensions.
	\caption{LTC dynamics with and without demand side support. Time constant $T = 1$.}
	\label{fig:dynamics2}
\end{figure}
